Revisiting the Onsets and Frames Model with Additive Attention

Recent advances in automatic music transcription (AMT) have achieved highly accurate polyphonic piano transcription results by incorporating onset and offset detection. The existing literature, however, focuses mainly on the leverage of deep and complex models to achieve state-of-the-art (SOTA) accuracy, without understanding model behaviour. In this paper, we conduct a comprehensive examination of the Onsets-and-Frames AMT model, and pinpoint the essential components contributing to a strong AMT performance. This is achieved through exploitation of a modified additive attention mechanism. The experimental results suggest that the attention mechanism beyond a moderate temporal context does not benefit the model, and that rule-based post-processing is largely responsible for the SOTA performance. We also demonstrate that the onsets are the most significant attentive feature regardless of model complexity. The findings encourage AMT research to weigh more on both a robust onset detector and an effective post-processor.

==> jyun-mod/abstract.tex <==
\jm{Recent advances in automatic music transcription (AMT) have achieved highly accurate polyphonic piano transcription results by incorporating onset and offset detection. The existing literature, however, focuses mainly on the leverage of deep and complex models to achieve state-of-the-art (SOTA) accuracy, without understanding model behaviour.
In this paper, we conduct a comprehensive examination of Onsets-and-Frames model, and pinpoint the essential components responsible for a decent accuracy of AMT. 
This is achieved through exploitation of a modified additive attention mechanism.
The experimental results suggest that the attention mechanism beyond a moderate temporal context does not benefit the model, and that rule-based post-processing is largely responsible for the SOTA performance.
We also demonstrate that the onsets are the most significant attentive feature regardless of model complexity.
The findings encourage AMT research to weigh more on both a robust onset detector and an effective post-processor.}

==> jyun-mod/introduction-1.tex <==
\jm{Automatic music transcription (AMT) has been a crucial task in music information retrieval (MIR) that underlies a variety of important applications, such as turning a mass of audio data to an indexable format which enables queries based on musical structure~\cite{cuthbert2010music21}, converting the audio to a symbolic dataset taken as the input for music generation~\cite{huang2020pop, herremans2017functional} or music accompaniments to play along with~\cite{magalhaeschordify}.}



==> jyun-mod/introduction-2.tex <==
\jm{Existing literature has been focusing on extending network capacity to achieve state-of-the-art (SOTA) transcription accuracy.
This includes fully convolutional neural networks~\cite{springenberg2014striving}, hybrid convolutional and recurrent neural networks~\cite{Sigtia2015AnEN}, and convolutional sequence-to-sequence models~\cite{Sigtia2015AnEN}.
In parallel to increasing model complexity, incorporating onset~\cite{Hawthorne2017OnsetsAF} and offset~\cite{kim2019adversarial, kelz2019deep} detection, and leveraging a large dataset~\cite{hawthorne2018enabling} for model training are also shown to improve the performance.
Despite the development, the components responsible for the superior performance remain unclear. 
To the best of our knowledge, only Kelz \textit{et al.} have attempted to explain AMT models using invertible neural networks~\cite{Kelz18}.
Although the work hints towards how the model possibly captures the notion of musical notes, it does not provide further insights on the relevant features for transcription.}

==> jyun-mod/introduction-3.tex <==
\jm{The main proposition of this paper is to elucidate the underlying components that lead to a performant AMT model.
We aim to anlayze and identify 1) the feature on which Onsets and Frames~\cite{Hawthorne2017OnsetsAF} relies the most to achieve the SOTA accuracy; 2) the length of temporal context with which the classifier obtains the most gain in accuracy; and 3) the interplay between the temporal information and different model constitutions.
These are achieved by using the additive attention~\cite{Bahdanau2015NeuralMT} which is slightly modified to facilitate our analysis.
The results indicate that, although temporal information is helpful, the length of the attentive context has to be limited in order to obtain a superior performance. 
Additionally, given a decent accuracy of onset prediction, the rule-based inference model accounts for the majority of the improvement in terms of note-wise transcription accuracy.
Our findings shed lights on promising avenues of research for improving AMT systems.}


==> jyun-mod/introduction-4.tex <==
\jm{We structure the rest of the paper as follows.
The background relevant to Onsets and Frames is provided in Section~\ref{sec:related_works}.
In Section~\ref{sec: proposed_work}, we propose the framework for analyzing Onsets and Frames, using the modified additive attention~\cite{Bahdanau2015NeuralMT} which serves as the probing tool.
Section~\ref{sec: experiment} elaborates the experimental setups including the dataset, model parameters, and the evaluation methods.
We thoroughly discuss the experimental results in Section~\ref{sec:result}, and conclude the paper in Section~\ref{sec:conclusion}.
}
